Non-Linear behavior of the Electron Cyclotron Drift Instability and the Suppression of Anomalous Current

We present results of one-dimensional collisionless simulations of plasma turbulence and related anomalous electron current of the Electron Cyclotron Drift Instability (ECDI). Our highly resolved, long-term simulations of xenon plasma in the magnetic field performed with the WarpX particle-in-cell (PIC) code show several intermediate non-linear stages before the system enters a stationary state with significantly increased electron temperature and a finite level of energy in the electrostatic fluctuations. In early and intermediate non-linear stages, the fluctuations are driven by the electron cyclotron resonances gradually shifting from higher ($m>1$) modes to the fundamental $m=1$ resonance. Enhanced resonant growth is observed from the point when the cyclotron $m=1$ mode coincides with the most unstable ion-acoustic mode. In the final stage, the anomalous electron current existing in intermediate stages is quenched to zero. Following this quenching, our simulations reveal a transition from ECDI-driven dynamics to saturated ion-acoustic turbulence. The modification of the electron and ion distribution functions and their roles in the non-linear developments and saturation of the instability are analyzed at different non-linear stages. The non-linear development of ECDI driven by the $\mathbf{E} \times \mathbf{B}$ electron drift from the applied current and the ECDI driven by the ion beam perpendicular to the magnetic field are compared and characterized as two perspectives of the instability, observed through different Doppler-shifted frames. An extension of this work incorporating full the dynamics of magnetized ions for ECDI driven by a hydrogen ion beam is shown to develop full beam inversion, with the periodic bursts of growth-saturation cycles of ECDI.

==> name.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{FIGURES/FIG_4A.pdf}
%     \includegraphics[width=0.9\linewidth]{FIGURES/FIG_4B.pdf}
%     \includegraphics[width=0.9\linewidth]{FIGURES/FIG_4C.pdf}
%     \includegraphics[width=0.9\linewidth]{FIGURES/FIG_4D.pdf}
%     \includegraphics[width=0.9\linewidth]{FIGURES/FIG_4E.pdf}
%     \caption{The snapshots of the evolution of four quantities shown for five different timeframes. Column 1: Ion phasespace in the z-direction, Column 2: Ion distribution function $\mathit{\tilde{f_i}}$ as described in Section \ref{}, Column 3: Electron phasespace in the z-direction, and Column 4: Electron distribution function $\mathit{\tilde{f_e}}$ as described in Section \ref{}.}
%     \label{fig:combined}
% \end{figure*}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5A.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5B.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5C.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5D.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5E.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5F.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_5G.pdf}
%     \caption{Two-dimensional fourier transform of electric field between four different timeframes. (a) $\mathit{E_z}$ from 0 < t < $\mathit{T_1}$, (b) $\mathit{E_z}$ from $\mathit{T_1} < t < \mathit{T_3}$, (c) $\mathit{E_z}$ from $\mathit{T_3}$ < t < $\mathit{T_5}$, and (d) $t >> \mathit{T_5}$} 
%     \label{fig:combined}
% \end{figure*}




% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_PowSpecA.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_PowSpecB.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_PowSpecC.pdf}
%     \includegraphics[width=0.48\linewidth]{FIGURES/FIG_PowSpecD.pdf}
%     \caption{Power spectrum from $0 < t < T_3$.}
%     \label{fig:power_spectrum}
% \end{figure*}

% \begin{figure*}
% \centering
% \begin{subfigure}[b]{0.48\textwidth}
% \centering
% \includegraphics[width=\textwidth]{FIGURES/FIG_PowSpecA.pdf}
% \caption{$y=x$}
% \label{fig:y equals x}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.48\textwidth}
% \centering
% \includegraphics[width=\textwidth]{FIGURES/FIG_PowSpecB.pdf}
% \caption{$y=3\sin x$}
% \label{fig:three sin x}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.48\textwidth}
% \centering
% \includegraphics[width=\textwidth]{FIGURES/FIG_PowSpecC.pdf}
% \caption{$y=5/x$}
% \label{fig:five over x}
% \end{subfigure}
% \caption{Three simple graphs}
% \label{fig:three graphs}
% \end{figure*}


% \begin{figure*}[htbp]
%     %\centering
%     \includegraphics[width=0.49\linewidth]{FIGURES/FIG_6A.pdf}
%     \includegraphics[width=0.49\linewidth]{FIGURES/FIG_6B.pdf}
%     \includegraphics[width=0.49\linewidth]{FIGURES/FIG_6C.pdf}
%     \caption{The depiction of the non-linear resonance between the ion-acoustic branch and m = 1 ECDI mode for three different scenarios : (a) $E = 20000 V/m , B = 200 G$, (b) $E = 20000 V/m , B = 250 G$, (c) $E = 16000 V/m , B = 200 G$.}
%     \label{fig:figure3}
% \end{figure*}

% \begin{figure}[h]
%   \centering
%    \includegraphics[width=\linewidth]{FIGURES/FIG_7.pdf}
%    \caption{\label{fig:ion} Time evolution of the cross field electron mobility as defined in Eq. \ref{} for Case 1A.}
% \end{figure}

% \begin{figure*}[ht]
%   \centering
%    \includegraphics[width=0.8\linewidth]{FIGURES/FIG_8.pdf}
%    \caption{\label{fig:ion} Time evolution of (a) Temperature $\mathit{T_{ez}}$, and (b) Cross field mobility for different virtual axial length (VAL) models. The simulations are performed with VAL ($\mathit{L_x} = 1 \, cm, 2 \, cm, 4 \, cm, 6 \, cm, \, and \, 12 \, cm.$)}
% \end{figure*}
